Deploying ZKP Frameworks with Real-World Data: Challenges and Proposed Solutions

Zero-knowledge proof (ZKP) frameworks have the potential to revolutionize the handling of sensitive data in various domains. However, deploying ZKP frameworks with real-world data presents several challenges, including scalability, usability, and interoperability. In this project, we present Fact Fortress, an end-to-end framework for designing and deploying zero-knowledge proofs of general statements. Our solution leverages proofs of data provenance and auditable data access policies to ensure the trustworthiness of how sensitive data is handled and provide assurance of the computations that have been performed on it. ZKP is mostly associated with blockchain technology, where it enhances transaction privacy and scalability through rollups, addressing the data inherent to the blockchain. Our approach focuses on safeguarding the privacy of data external to the blockchain, with the blockchain serving as publicly auditable infrastructure to verify the validity of ZK proofs and track how data access has been granted without revealing the data itself. Additionally, our framework provides high-level abstractions that enable developers to express complex computations without worrying about the underlying arithmetic circuits and facilitates the deployment of on-chain verifiers. Although our approach demonstrated fair scalability for large datasets, there is still room for improvement, and further work is needed to enhance its scalability. By enabling on-chain verification of computation and data provenance without revealing any information about the data itself, our solution ensures the integrity of the computations on the data while preserving its privacy.

==> tex/sections/architecture.tex <==
\section{Architecture}
Figure~\ref{fig:architecture} illustrates the overall architecture of the Fact Fortress framework. Data providers securely store their sensitive data and set data access policies, while data analyzers request access to the data based on these policies. Alternatively, data analyzers can delegate computation on their behalf to Fact Fortress, which returns the zero-knowledge proof and the computation result directly to them.

Data analyzers can publish the result of the computation along with the proof, which anyone can verify. When uploading a proof to Fact Fortress (via QR code or JSON), our platform verifies that:
\begin{enumerate}
\item The proof was generated by the function claimed by the researcher.
\item The data used to generate the proof has not been tampered with and comes from the data providers claimed by the researcher.
\item The claimed result is the correct result of the function applied to the data.
\end{enumerate}


\begin{figure*}[h]
    \centering
    \includegraphics[width=1\textwidth]{img/fortress_overview.pdf}
    \caption{Proposed ZKP framework}
    \label{fig:architecture}
\end{figure*}


==> tex/sections/implementation.tex <==
\section{Implementation on Ethereum}

In this section, we provide a detailed description of the technical implementation of Fact Fortress on the Ethereum blockchain. We discuss the various components of the system, including the circuit generator, the proof generator, and the on-chain verifier, and explain how they work together to provide a secure and efficient solution for fact-checking.

Additionally, we highlight the system's current limitations and discuss potential areas for improvement.

\subsection{Off-Chain Layer (Circuits)}

Several circuits have been implemented for this project. In that context, we use Noir, a domain-specific language for SNARK proving systems~\cite{noir}
created by the developers of the Aztek Network
% \footnote{\url{https://aztec.network/}}
. Noir compiles circuits into Abstract Circuit Intermediate Representations (ACIR) compatible with different SNARK-based proving systems. We have used the default one for this project: the PLONK SNARK prover Barretenberg.

\subsubsection{Circuit 1. Toy Circuit: Validation of Schnorr Signatures}

The first circuit we implemented ensures a data provider has signed data. This circuit takes a public key generated on the Grumpkin curve (an elliptic curve based on BN254~\cite{gabizon_williamson_walton-pocock})
 as public input, the hashed private data, and its associated signature as private inputs. It then verifies that the signature corresponds to the public key using the following Rust function
% \footnote{\url{https://noir-lang.org/standard_library/cryptographic_primitives/schnorr/\#schnorrverify_signature}. Note: the official documentation has been updated to reflect our observation that Noir cannot verify default Schnorr signatures. See: \url{https://github.com/noir-lang/noir/issues/1141}}
.

\begin{footnotesize}
\begin{verbatim}
fn verify_signature(
    _public_key_x: Field, 
    _public_key_y: Field, 
    _signature: [u8; 64], 
    _message: [u8]
) -> Field
\end{verbatim}
\end{footnotesize}

Thanks to this circuit, once proof of provenance is generated, a verifier can ensure that the data provider has signed the hash. This circuit is presently used in our end-to-end solution; we will replace it soon with auto-generated circuits that embeds the proof of provenance (see above).

\subsection{Solidity Smart Contracts}

To date, we have implemented three Solidity smart contracts. 

The first contract\footnote{\url{https://github.com/pierg/fact-fortress-dapp/blob/main/contracts/factFortress.sol}} 
is the entry point of the solution. It notably interacts with two other contracts described below that grant and revoke permissions (to perform on-chain actions and access online data). It also interacts with the validator contracts to verify public inputs and proofs submitted by verifiers.



The second and third contracts\footnote{ERC-721 smart contracts:\\\url{https://github.com/pierg/fact-fortress-dapp/blob/main/contracts/dataProvidersNFTs.sol}, \url{https://github.com/pierg/fact-fortress-dapp/blob/main/contracts/dataAnalystsNFTs.sol}}
implement the ERC-721 Non-Fungible Token standard~\cite{eip721}
to manage NFTs. These NFTs are used as \textit{decentralized} authorization tokens. They allow data providers to update their public keys on the blockchain and enable data analyzers to access the data.


We have also improved an existing mechanism from the Noir library to generate smart contracts. Noir offers two ways to generate the verifier smart contract: via command line (\texttt{nargo codegen-verifier}) or programmatically, via a TypeScript library (\texttt{@noir-lang}). We identified that these approaches generate different smart contracts. After having assessed them, we have determined that generating the verifier smart contract programmatically was more optimal—while imperfect (see Section \ref{sec:limitations})—for our use case, to create the verifier contracts.

The fourth contract, generated in these conditions, verifies the proof of provenance using the Schnorr signature verification circuit. Additional validator contracts—notably verifying the risk score function—are scheduled to be deployed. 

These smart contracts are currently deployed on Ganache, an Ethereum blockchain simulator for development purposes~\cite{Ganache}.


\subsection{Current Limitations} 
\label{sec:limitations}

We have identified and addressed several shortcomings affecting Noir. Issues were expected, as this language is still experimental. \newline

\noindent
\textbf{Transient Blocking Issue Affecting the Programmatic Compilation of Circuits}


The circuit generator is currently not fully connected to the rest of the application. The issue comes from the fact that our autogenerated contracts, which use recent features offered by Noir (v0.4.0 and above), are not programmatically compilable due to a bug affecting the Noir WASM module, as we explain below. In other words, while the most recent version of the \texttt{nargo} command can compile them, our application presently lacks this ability.

Because the circuits are compiling off-chain, we are confident about the technical feasibility of achieving a full integration in the short term. \newline

\noindent
\textbf{Overcoming Technical Limitations From Noir}



First, \texttt{@noir-lang} a WebAssembly (WASM) module, written in Rust, to compile the circuits.
% \footnote{\url{https://github.com/noir-lang/noir_wasm}}
Using WASM \textit{modules} allows the Noir developers to maintain the compiler in Rust while offering the possibility of implementing applications (the \textit{hosts}—in WebAssembly terminology) that call this compiler in other languages. The host function provides the path to the circuit definition to the WASM module, which compiles it and returns the compiled circuit to the host. This decoupling between the host and the module has led to difficulties in this project for two main reasons. (a) We could not programmatically compile some contracts, while the CLI command, \texttt{nargo}, could; the WASM module was indeed outdated. (b) Compiler errors from the \texttt{@noir-lang} WASM modules are hard to analyze, as demonstrated by this example~\cite{github1175}, where a runtime error, from the host perspective, is caused by an obscure circuit compilation error, from the module perspective.

% \begin{footnotesize}
% \begin{verbatim}
% RuntimeError: unreachable
% at wasm://wasm/00a338b6:wasm-function[2495]:0x272def
% at wasm://wasm/00a338b6:wasm-function[1514]:0x259c66
% at wasm://wasm/00a338b6:wasm-function[1732]:0x265732
% at wasm://wasm/00a338b6:wasm-function[450]:0x1b303b
% at wasm://wasm/00a338b6:wasm-function[1671]:0x2626b4
% at wasm://wasm/00a338b6:wasm-function[1212]:0x241d6e
% \end{verbatim}
% \end{footnotesize}


Second, we noticed that the default smart contracts autogenerated by Noir to verify Schnorr signatures failed at compile or runtime. More precisely, contracts generated by the command line systematically reverted despite valid inputs. And contracts programmatically generated by (\texttt{@noir-lang}) were affected by a \texttt{Stack too deep} compiler error, as Noir generates a function referring to a number of variables larger than the EVM stack limit (limited to 16 slots). The issue was fixed by adding block scopes~\cite{github1133}, and Fact Fortress now uses this technique to make the verifier contracts compilable.

Third, and more problematically, the verifier smart contract functions generated by Noir only accept the serialized proof as a parameter, which contains public inputs as embedded bytes. In other words, these contracts do not allow to specify the public inputs associated with a proof. To overcome this issue, an extractor and a public input verifier had to be implemented in the main smart contract\footnote{See: \url{https://github.com/pierg/fact-fortress-dapp/blob/main/contracts/factFortress.sol\#L233-L287}}. Therefore, the main contract performs a pre-check on the public inputs before calling the relevant verifier smart contract with the actual proof.\newline

The Noir language represents a valuable resource for simplifying the implementation of circuits. Despite its experimental nature and occasional bugs, our experience shows that Noir offers significant advantages for circuit generation, including ease of use and increased efficiency. These benefits can be considerable when time and resource constraints are essential.

==> tex/sections/technical.tex <==


\subsection{General Approach}






The goal of Zero-Knowledge Proof is to prove the truth of a statement without revealing any information that could compromise the privacy or security of the data. In our case, we want to prove that we know a specific value $w$ from a trusted authority $A$ such that $f(w)=y$, where $f$ is a function that takes $w$ as input and produces $y$ as output. The value $w$ is sensitive and needs to be protected, while $y$ is the result of a computation that we want to prove without revealing the input value $w$.

With Zero-Knowledge Proof, we are able to prove the truth of the statement without disclosing any information about $w$. Specifically, the proof will certify that:

\begin{enumerate}
\item The data $w$ came from the trusted authority $A$.
\item The data $w$ has not been tampered with before applying the function $f$.
\item The result $y$ is the output of the function $f$ applied to the data $w$.
\end{enumerate}

To achieve this, the prover generates a proof of the statement, and the verifier checks the proof without requiring any knowledge of the sensitive data $w$. Both the prover and verifier must agree on the function $f$ to be executed on the data $w$, and the verifier must be convinced that the proof is valid.


Figure~\ref{fig:zkp-blocks} shows the various entities involved in the proof of a generic claim in zero-knowledge. In the following we describe the main entities involved and their interaction.

\textbf{Authority A}
Let $A$ be an authority (e.g. a hospital) that possesses some sensitive data $w$. Let $d_A$ and $Q_A$ denote the private and public keys of $A$, respectively, which have been generated by some elliptic curve cryptography (ECC) generator. To sign and protect the authenticity of $w$, $A$ produces the hash of $w$, i.e., $H_w$, and signs it with its private key $d_A$ using the Elliptic Curve Digital Signature Algorithm (ECDSA).

\textbf{Claim}
The public claim is that $y$ is the result of applying $f$ to some sensitive data $w$, and that $w$ has been generated by $A$. In order to produce the proof, we must encode the function $f$ as an arithmetic circuit $C$.

\textbf{Trusted Setup}
The trusted setup procedure takes as input the circuit $C$ representing the function on $w$ and some random parameter $\lambda$, and produces $S_p$ and $S_v$, which are the public parameters for the prover and the verifier, respectively. The parameter $\lambda$ must be destroyed after its use, as if the prover gains knowledge of it, it can generate false proofs.


\textbf{Prover}
The prover 





\subsubsection{The Prover}

The prover's goal is to convince the verifier that the statement is true, without revealing any information about $w$. To do this, the prover generates a proof using the sensitive data $w$, the function $f$, and the public parameters agreed upon with the verifier. The proof must be constructed in a way that allows the verifier to check its validity without any knowledge of $w$.

\subsubsection{The Verifier}

The verifier's goal is to check the validity of the proof provided by the prover, without requiring any knowledge of the sensitive data $w$. To do this, the verifier uses the public parameters agreed upon with the prover, and checks that the proof satisfies a set of mathematical criteria that guarantee the truth of the statement. If the proof is valid, the verifier accepts the statement as true without gaining any knowledge of $w$.



\textbf{Key Generation:}

\begin{itemize}
\item[] \textbf{Input:} None
\item[] \textbf{Output:} Private key $d$ and public key $(Q_x, Q_y)$
\end{itemize}

\textbf{Message Digest:}

\begin{itemize}
\item[] \textbf{Input:} Message $w$
\item[] \textbf{Output:} Message digest or hash $H_w$
\end{itemize}

\textbf{Signing:}

\begin{itemize}
\item[] \textbf{Input:} Private key $d$, message digest $H_w$
\item[] \textbf{Output:} Signature $(r, s)$
\item[] \textbf{Procedure:}
\begin{enumerate}
\item Generate a random number $k$
\item Calculate the point $(x_1, y_1) = k \cdot G$, where $G$ is the generator point of the elliptic curve
\item Calculate $r = x_1 \bmod n$, where $n$ is the order of $G$
\item Calculate $s = k^{-1} (H_w + dr) \bmod n$
\item Return the signature $(r, s)$
\end{enumerate}
\end{itemize}

\textbf{Verification:}

\begin{itemize}
\item[] \textbf{Input:} Public key $(Q_x, Q_y)$, message $w$, signature $(r, s)$
\item[] \textbf{Output:} Boolean value indicating whether the signature is valid
\item[] \textbf{Procedure:}
\begin{enumerate}
\item Calculate the message digest or hash $H_w$
\item Calculate $w = s^{-1} \bmod n$ and $u_1 = H_w \cdot w \bmod n$
\item Calculate $u_2 = r \cdot w \bmod n$
\item Calculate the point $(x_1, y_1) = u_1 \cdot G + u_2 \cdot (Q_x, Q_y)$
\item If $r = x_1 \bmod n$, the signature is valid, otherwise it is invalid.
\end{enumerate}
\end{itemize}







In many scenarios, it is necessary to collect some digitally signed data, process it, and publish the result of the computation in a way that preserves the privacy and security of the data. Specifically, a zero-knowledge proof can be used to demonstrate that:

\begin{enumerate}
    \item The data is authentic, i.e., it has been digitally signed by a trusted party.
    \item The data has not been tampered with during the computation.
    \item The result published is the actual result of the computation performed on the data.
\end{enumerate}

This approach ensures that the sensitive data remains confidential, while still allowing for the publication of important results derived from it.

Let 

Here is a protocol that uses Zero Knowledge Proof (ZKP) and ECDSA for the authentication of "x" and the verification of "y".

Assume we have an elliptic curve group G and a trusted agency who holds the private key k and the public key P, and produces the secret witness x. Also assume we have a function $f(x)$ that produces y. Further, let R be a randomly generated point on the curve, and H be a hash function.

\begin{enumerate}
    \item The researcher generates a random value $r$ and computes $A = rP$, and $B = rR$.
    \item The researcher sends $A$ and $B$ to the trusted agency.
    \item The trusted agency sends a challenge $e$ to the researcher, which is a hash of $A$, $B$, and the function $f$.
    \item The researcher computes $s = r + ex \mod n$, where $n$ is the order of the curve, and sends $s$ to the trusted agency.
    \item The trusted agency verifies the proof by computing $A' = sP - eB$ and checking if $A' = A$. If it is equal, then the researcher has demonstrated knowledge of x without revealing it.
    \item To verify that $y = f(x)$, the researcher sends $(y, R)$ to the verifier.
    \item The verifier generates a random value $u$ and computes $A = uP + yH(R)$, and $B = uR$. The verifier sends $A$ and $B$ to the researcher.
    \item The researcher sends a challenge $e$ to the verifier, which is a hash of $A$, $B$, and the function $f$.
    \item The verifier computes $s = u + ex \mod n$ and sends $s$ to the researcher.
    \item The researcher verifies the proof by computing $A' = sP - eB$ and checking if $A' = A$. If it is equal, then the verifier has demonstrated knowledge of $x$, and $y = f(x)$.
\end{enumerate}

In this protocol, the ZKP ensures that the researcher is not tampering with the witness $x$ or trying to take any shortcuts in computing $y$. The ECDSA ensures that the trusted agency and verifier can verify the proofs without the knowledge of the witness $x$.





\subsection{General Approach}

\noindent A trusted agency $A_1$ having public and private keys $(pk_{A_1}, sk_{A_1})$ produce some data $x$. 
A researcher $R$ with keys $(pk_{R}, sk_{R})$ produces $y=f(x)$ and a proof $\pi$ that shows in zero knowledge (i.e. without revealing $x$) that $x$ comes from $A_1$ and has not been tampered, and that $y=f(x)$. 
A verifier $V$ verifies the proof $\pi$. 

\noindent \textbf{Protocol Steps:}

\begin{enumerate}[label=X\arabic*.,ref=X\arabic*]
    
    \item $A_1$ publishes $pk_{A_1}$ for verification purposes.
    
    \item $R$ generates a random number $r$ and computes $z = f(r)$. 

    \item $R$ uses the private key $sk_{R}$ to sign $z$ using ECDSA, producing $\sigma = Sign_{sk_{R}}(z)$.

    \item $R$ sends $(y,r,\sigma)$ to $V$ along with the following zero knowledge proof $\pi$:
    
    \begin{enumerate}[label=X\arabic*.,ref=X\arabic*]
        \item $R$ computes $c = H(pk_{A_1}, y, z)$ where $H$ is a cryptographic hash function. 
        
        \item $R$ computes $s = r + c \cdot sk_{R} \pmod{q}$ where $q$ is the order of the elliptic curve used in ECDSA.
        
        \item $R$ sends $c$ and $s$ to $V$.
        
        \item $V$ verifies that $sG = r\cdot G + c\cdot pk_{R}$ where $G$ is the generator point of the elliptic curve used in ECDSA.
        
        \item $V$ computes $z' = f(sG - c\cdot pk_{A_1})$. 
        
        \item $V$ checks that $c = H(pk_{A_1}, y, z')$ and accepts the proof if the check passes.
    \end{enumerate}
    
    \item If the proof $\pi$ is accepted, $V$ can trust that $y=f(x)$ without knowing $x$, and that $x$ came from $A_1$ and was not tampered. 
\end{enumerate}





Here is a sample sequence diagram in LaTeX using the `pgf-umlsd` package:


\begin{sequencediagram}
    \newthread{A}{Agency $A_1$}
    \newinst[2]{R}{Researcher $R$}
    \newinst[2]{V}{Verifier $V$}
    \begin{call}{A}{Publish $pk_{A_1}$}{V}{}
    \end{call}
    \begin{sdblock}{Loop}{For each data $x$}
        \begin{call}{A}{Produce $x$}{R}{}
        \end{call}
        \begin{call}{R}{Compute $y=f(x)$}{R}{}
        \end{call}
        \begin{call}{R}{Generate $r$}{R}{}
        \end{call}
        \begin{call}{R}{Compute $z=f(r)$}{R}{}
        \end{call}
        \begin{call}{R}{Sign $z$ with $sk_R$}{R}{$\sigma = Sign_{sk_R}(z)$}
        \end{call}
        \begin{call}{R}{Send $(y,r,\sigma)$\\and $\pi$ to $V$}{V}{}
            \begin{callself}{V}{Verify proof $\pi$}{}
            \end{callself}
        \end{call}
    \end{sdblock}
\end{sequencediagram}

